Multiplier Optimization via E-Graph Rewriting

Multiplier circuits account for significant resource usage in datapath-dominated circuit designs, and RTL designers continue to build bespoke hand-crafted multiplication arrays for their particular application. The construction of an optimized multiplier presents trade-offs between pre-processing to generate a smaller array and array reduction. A data structure known as an e-graph has recently been applied to datapath optimization, where the e-graph's ability to efficiently explore trade-offs has been shown to be crucial. We propose an e-graph based rewriting framework to construct optimized multiplier circuits. Such a framework can express alternative multiplier representations and generate customized circuit designs. We demonstrate that the proposed tool, which we call OptiMult, can reduce the latency of a squarer by up to 46% and reduce the latency of a standard multiplier by up to 9% when compared against logic synthesis instantiated components.

==> array1.tex <==
\[\begin{array}{
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
}
\hline
7 & 6 & 5 & 4 & 3 & 2 & 1 & 0 \\
$x_3 y_0$ & $x_3 y_0$  & $x_3 y_0$ & $x_3 y_0$ & $x_3 y_0$ & $x_2 y_0$ & $x_1 y_0$ & $x_0 y_0$ \\
$x_3 y_1$ & $x_3 y_1$  & $x_3 y_1$ & $x_3 y_1$ & $x_2 y_1$ & $x_1 y_1$ & $x_0 y_1$ & \\
$x_3 y_2$ & $x_3 y_2$  & $x_3 y_2$ & $x_2 y_2$ & $x_1 y_2$ & $x_0 y_2$ & \\
$\overline{x_3} y_3$ & $\overline{x_3} y_3$ & $\overline{x_2} y_3$ & $\overline{x_1} y_3$ & $\overline{x_0} y_3$ & & \\
                   &                    &                    &                    &               $y_3$\\
\end{array}\]

==> array2.tex <==
\[\begin{array}{
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
}

7 & 6 & 5 & 4 & 3 & 2 & 1 & 0 \\
\hline 
  &                             1 &                  1 &                  1 &               1\\
1 & 1  & 1 & 1 & $\overline{x_3 y_0}$ & $x_2 y_0$ & $x_1 y_0$ & $x_0 y_0$ \\
1 & 1  & 1 & $\overline{x_3 y_1}$ & $x_2 y_1$ & $x_1 y_1$ & $x_0 y_1$ & \\
1 & 1  & $\overline{x_3 y_2}$ & $x_2 y_2$ & $x_1 y_2$ & $x_0 y_2$ & \\
1 & $\overline{\overline{x_3} y_3}$ & $\overline{x_2} y_3$ & $\overline{x_1} y_3$ & $\overline{x_0} y_3$ & & \\
  &                               &                    &                    &               $y_3$
  
\end{array}
\]

==> array3.tex <==
\[
\begin{array}{
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
>{\centering\arraybackslash}p{2em}<{}
}
7 & 6 & 5 & 4 & 3 & 2 & 1 & 0 \\
\hline 
 &   &  & $y_3$ & $\overline{x_3 y_0}$ & $x_2 y_0$ & $x_1 y_0$ & $x_0 y_0$ \\
 &   &  & $\overline{x_3 y_1}$ & $x_2 y_1$ & $x_1 y_1$ & $x_0 y_1$ & \\
 &   & $\overline{x_3 y_2}$ & $x_2 y_2$ & $x_1 y_2$ & $x_0 y_2$ & \\
1 & $\overline{\overline{x_3} y_3}$ & $\overline{x_2} y_3$ & $\overline{x_1} y_3$ & $\overline{x_0} y_3$ & & \\
 
\end{array}
\]

==> signed_array_reduction.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{\columnwidth}
         \centering
            \input{array1}
         \caption{Initial AND array, including sign extension.}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\columnwidth}
         \centering
            \input{array2}
         \caption{Deploying the ``repeated-bit'' rewrite.}
         \label{fig:repeated-bit}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\columnwidth}
         \centering
            \input{array3}
         \caption{Reducing constant bits using Boolean reduction.}
         \label{fig:final-array}
     \end{subfigure}
        \caption{Stages of signed array optimization, as described in~\cite{Ercegovac2004DigitalArithmetic}. We use $\overline{a}$ to denote inversion of a single bit, $a$. \scom{Probably remove this diagram - not central and could be described in words}}
        \label{fig:array-optimizations}
\end{figure}

==> stage_table.tex <==
\begin{table*}
    \centering
    \caption{Stages at which expressions are extracted, preventing the e-graph from continuously growing exponentially attempting to search the total space}
    \label{tab:stages}
    \setlength\extrarowheight{2pt}
    \rowcolors{2}{gray!25}{white}
    \begin{tabular}{|c|c|c|}
        \hline
         Start Expression Name & End Expression Name & Iterative \\
         \hline
         Multiplication expression & And array & No \\
         And array & Initial half and full adder placement & No \\
         Initial half and full adder placement & Complete adder placement & Yes \\
         Complete adder placement & Gate optimised expression & Yes \\    
        \hline     
    \end{tabular}
\end{table*}
